Keeping Pace with Ever-Increasing Data: Towards Continual Learning of Code Intelligence Models

Previous research on code intelligence usually trains a deep learning model on a fixed dataset in an offline manner. However, in real-world scenarios, new code repositories emerge incessantly, and the carried new knowledge is beneficial for providing up-to-date code intelligence services to developers. In this paper, we aim at the following problem: How to enable code intelligence models to continually learn from ever-increasing data? One major challenge here is catastrophic forgetting, meaning that the model can easily forget knowledge learned from previous datasets when learning from the new dataset. To tackle this challenge, we propose REPEAT, a novel method for continual learning of code intelligence models. Specifically, REPEAT addresses the catastrophic forgetting problem with representative exemplars replay and adaptive parameter regularization. The representative exemplars replay component selects informative and diverse exemplars in each dataset and uses them to retrain model periodically. The adaptive parameter regularization component recognizes important parameters in the model and adaptively penalizes their changes to preserve the knowledge learned before. We evaluate the proposed approach on three code intelligence tasks including code summarization, software vulnerability detection, and code clone detection. Extensive experiments demonstrate that REPEAT consistently outperforms baseline methods on all tasks. For example, REPEAT improves the conventional fine-tuning method by 1.22, 5.61, and 1.72 on code summarization, vulnerability detection and clone detection, respectively.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> section/related.tex <==
\section{Related work}\label{sec:related}

\subsection{Deep Learning for Code}
Deep learning techniques have been widely used to in many code intelligence tasks. % including code summarization, vulnerability detection and code clone detection. 
In this section, we introduce the code intelligence tasks covered in our work, including code summarization, vulnerability detection, and code clone detection. Besides, we also discuss the related work on pre-trained models of code.
%\hy{say something about code intelligence and Deep Learning for Code in general}

\textbf{Code Summarization}
is the task of automatically generating a short natural language description for the given source code. Recent researches in this field resort to deep learning techniques such as sequence-to-sequence models and achieve state-of-the-art performance. Iyer et al.~\cite{DBLP:conf/acl/IyerKCZ16} propose CODE-NN, the first deep-learning-based work in code summarization, which consist of a Long Short Term Memory (LSTM)~\cite{hochreiter1997long} and attention mechanism. Hu et al.~\cite{DBLP:conf/iwpc/HuLXLJ18} propose to integrate the code structure information through the structure-based traversal (SBT). Wei et al.\cite{DBLP:conf/kbse/Wei19} and Zhang et al.\cite{DBLP:conf/icse/ZhangW00020} further take advantages of the retrieved information to enable more informed code summarization. Ahmad  et al.~\cite{DBLP:conf/acl/AhmadCRC20} introduce Transformer for code summarization and achieve promising performance. Recently, more works~\cite{DBLP:conf/acl/WuZZ21,DBLP:journals/corr/abs-2202-06521,DBLP:conf/icse/TangSLGHZ022,10.1145/3522674} integrates code structure information into Transformer and get better performance on code summarization.

\textbf{Vulnerability Detection: } aims to detect whether there are vulnerabilities in the source code, which is crucial to defend a software system from cyberattacks~\cite{DBLP:journals/tosem/ZouZXLJY21,DBLP:conf/nips/ZhouLSD019}. \revise{Li et al.~\cite{DBLP:conf/ndss/LiZXO0WDZ18} propose VulDeePecker which employs BiLSTM for vulnerability detection. Devign~\cite{DBLP:conf/nips/ZhouLSD019} is proposed to learn the various vulnerability characteristics with a composite code property graph and graph neural network. Reveal \cite{reveal} {leverage} GGNN \cite{Method3} to model multiple code relationships from source code. Li et al.~\cite{IVDETECT} explore vulnerability explainability based on Graph Convolutional Network and propose IVDETECT.}

\textbf{Code Clone Detection}
is the task of which can help \revise{reduce the cost of software maintenance and prevent faults. Wei et al.~\cite{DBLP:conf/ijcai/WeiL17} propose CDLH to learn hash codes from the lexical and structural information. Zhao et al.~\cite{DBLP:conf/sigsoft/ZhaoH18} propose DeepSim which encodes the program’s control flow graph and data flow graphs into matrices to measure functional similarity. Yu et al.~\cite{DBLP:conf/iwpc/YuLCLXW19} propose TBCCD to detect semantic clones using tree-based convolutional neural network capturing both the lexical and structural information of code snippets.} Wang et al.~\cite{DBLP:journals/corr/abs-2002-08653}, propose FA-AST which augments
original ASTs with explicit control and data flow edges and achieve state-of-the-art performance.

%aims at retrieving semantic relevant code snippet for the given natural language query. Gu et al.~\cite{DBLP:conf/icse/GuZ018} first propose DCS which uses a deep neural network to encode method name, api sequence and tokens of the source code. Another work UNIF~\cite{DBLP:conf/sigsoft/CambroneroLKS019} propose to calculate the similarity through the hidden states encoded by the LSTM network. OCoR~\cite{DBLP:conf/kbse/ZhuSLXZ20} propose to leverage the overlapping between code and query to find semantically similar code. Recently, CDCS~\cite{DBLP:journals/corr/abs-2201-00150} investigate cross domain code search with meta learning. Another recent work~\cite{DBLP:conf/icse/SunFCTHZ22} propose to reduce the semantic gap between code natural language by  translating code snippets into natural language descriptions.

\textbf{Pre-trained model of code.}
\revise{Learning high-quality code representations is of vital importance for deep-learning-based code-related tasks. Recently, a number of pre-trained models for source code have been proposed and shown effective in many code intelligence tasks~\cite{DBLP:conf/emnlp/FengGTDFGS0LJZ20,DBLP:conf/iclr/GuoRLFT0ZDSFTDC21,DBLP:conf/emnlp/0034WJH21}. CodeBERT~\cite{DBLP:conf/emnlp/FengGTDFGS0LJZ20} is an encoder-only pre-trained model based on Masked language modeling and replaced token detection. GraphCodeBERT~\cite{DBLP:conf/iclr/GuoRLFT0ZDSFTDC21} further leverage code structure information by data flow graph. CodeT5~\cite{DBLP:conf/emnlp/0034WJH21} regards all the tasks as sequence to sequence paradigm with different task specific prefixes and achieve  state-of-the-art performance on a variety code intelligence tasks.}
